Search-based User Interest Modeling with Lifelong Sequential Behavior Data for Click-Through Rate Prediction

Rich user behavior data has been proven to be of great value for click-through rate prediction tasks, especially in industrial applications such as recommender systems and online advertising. Both industry and academy have paid much attention to this topic and propose different approaches to modeling with long sequential user behavior data. Among them, memory network based model MIMN proposed by Alibaba, achieves SOTA with the co-design of both learning algorithm and serving system. MIMN is the first industrial solution that can model sequential user behavior data with length scaling up to 1000. However, MIMN fails to precisely capture user interests given a specific candidate item when the length of user behavior sequence increases further, say, by 10 times or more. This challenge exists widely in previously proposed approaches. In this paper, we tackle this problem by designing a new modeling paradigm, which we name as Search-based Interest Model (SIM). SIM extracts user interests with two cascaded search units: (i) General Search Unit acts as a general search from the raw and arbitrary long sequential behavior data, with query information from candidate item, and gets a Sub user Behavior Sequence which is relevant to candidate item; (ii) Exact Search Unit models the precise relationship between candidate item and SBS. This cascaded search paradigm enables SIM with a better ability to model lifelong sequential behavior data in both scalability and accuracy. Apart from the learning algorithm, we also introduce our hands-on experience on how to implement SIM in large scale industrial systems. Since 2019, SIM has been deployed in the display advertising system in Alibaba, bringing 7.1\% CTR and 4.4\% RPM lift, which is significant to the business. Serving the main traffic in our real system now, SIM models user behavior data with maximum length reaching up to 54000, pushing SOTA to 54x.

==> ch_abstract.tex <==
readme


==> ch_exp_pq.tex <==
\section{Experiments}
In this section, we present our experiments in detail, including
datasets, experimental setup, model comparison
and the corresponding analysis. The proposed search model is compared with several state-of-art works on two public dataset and one industrial dataset as shown in table \ref{table:Statistics}. Experiment result demonstrate the effectiveness of proposed approach on long-term model interest modeling. %, with which we wish to help advance the community.  

\subsection{Datasets}
Model comparisons are conducted on two public datasets as well as an industrial dataset collected from online display advertising system of Alibaba. Table \ref{table:Statistics} shows the statistics of all datasets.  

\begin{table}[]
%\setlength{\belowcaptionskip}{-1cm}
\caption{Statistics of datasets used in this paper.}
\small
\centering
\begin{threeparttable}
\begin{tabular}{lcccc}
\toprule
    Dataset       & Users & Items\tnote{a} & Categories & Instances \\ \midrule
Amazon(Book). & 75053 & 358367 & 1583 & 150016 \\ 
Taobao. & 7956431 & 34196612 & 5597 & 7956431 \\
Industrial.  & 0.29 billion & 0.6 billion & 100,000 & 12.2 billion \\ 
\bottomrule
\end{tabular}
			\begin{tablenotes}%[para,flushleft]
	        \item[a] For industrial dataset, items refer to be the advertisement.
		    \end{tablenotes}
 \end{threeparttable}
\label{table:Statistics}
\end{table} 

\textbf{Amazon Dataset\footnote{http://jmcauley.ucsd.edu/data/amazon/}} is composed of product reviews and metadata from Amazon . We use the \textsl{Books} subset of Amazon dataset which contains 75053 users, 358367 items and 1583 categories. For this dataset, we regard reviews as one kind of interaction behaviors, and sort the reviews from one user by time. The average behavior sequence length of amazon book dataset is "500". We split the recent 100 user behaviors as short-term user sequential features and recent 900 user behaviors  as long-term user sequential features. These pre-processing method has been widely used in related works.

\textbf{Taobao Dataset} is a collection of user behaviors from Taobao's recommender system. The dataset contains several types of user behaviors including click, purchase, etc.. It contains user behavior sequences of about eight million users. We take the click behaviors for each user and sort them according to time in an attempt to construct the behavior sequence. Assuming there are T behaviors of user u, we use the former T-1 clicked products as features to predict whether users will click the $T$-th product. The behavior sequence is truncated at length 1000.  The dataset is preparing to publish.

%is a collection of user behaviors from Taobao's recommender system \cite{Han2018Learning}. The dataset contains several types of user behaviors including click, purchase, etc. It contains user behavior sequences of about one million users. We take the click behaviors for each user and sort them according to time in an attempt to construct the behavior sequence. Assuming there are T behaviors of user u, we use the former T-1 clicked products as features to predict whether users will click the $T$-th product. The behavior sequence is truncated at length 200.  

\textbf{Industrial Dataset} is collected from online display advertising system of Alibaba. Samples are constructed from impression logs, with' click' or 'not' as label. Training set is composed of samples from past 49 days and test set from the following day, a classic setting for industrial modeling. In this dataset, user behavior feature in each day's sample contains historical behavior sequences from the preceding $180$ days. Thirty percent samples is over ten thousands length of behaviors.


\subsection{Competitors and experiment setup}
We compare SIM with mainstream CTR prediction models as follow. 
\begin{itemize}
        \item{\it \textbf{DIN}} is an early work for user behavior modeling which proposes to soft-search user behaviors w.r.t. candidates.          
		\item{\it \textbf{Long-term DIN}} is DIN add user's longterm behavior sequences with sum-pooling, so that we can compare model performance fairly on long-term user interest.
		\item{\it \textbf{MIMN}} which has ingeniously designed model architecture to capture long-term user interest achieves state-of-art performance. 
		\item{\it \textbf{SIM}} is the method proposed in this paper
		\item{\it \textbf{SIM with timestamp}}
\end{itemize}


\textbf{Experiment setup} we take the same experiment set up with related works[] so that the experiment results can be compared fairly. For all models, we use Adam solver.
We apply exponential decay with learning rate starting at 0.001
and decay rate of 0.9. Layers of FCN (fully connected network)
are set by $200 \times 100 \times 2$. The number of embedding dimension is set to be 16. And we take widely used AUC and loss as model performance measurement metrics.

\subsection{Results on Public Datasets}
\begin{table}
	\small
	\centering
	\caption{Model performance (AUC) on public datasets}\label{tab:public}
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{l c c}
			\addlinespace
			\toprule
			Model        & Taobao (mean $\pm$ std) & Amazon (mean $\pm$ std)\\
			\midrule		
			{\it DIN}~ & $ 0.9006 \pm 0.00094$  &  $ 0.7411 \pm 0.00185 $  \\
			{\it Long-term DIN}~    & $ 0.9066 \pm 0.00420$  &  $ 0.7420 \pm 0.00029 $  \\
			{\it MIMN}~    & $ 0.9081 \pm 0.00221$  &  $ 0.7481 \pm 0.00102 $  \\
			{\it SIM}~    & $\bm{0.9179 \pm 0.00325}$  &  $\bm{0.7593 \pm 0.00150}$  \\
			{\it SIM with timestamp}~    & $\bm{0.9179 \pm 0.00325}$  &  $\bm{0.7593 \pm 0.00150}$  \\
			\bottomrule
	\end{tabular}}
\end{table}
Table~\ref{tab:public} presents results of all the compared models. Compared with  DIN, all models taking in long-term user behavior features perform much better on AUC and log-loss. It demonstrates that the long-term user behavior is helpful for CTR prediction task. MIMN improves the performance of Longterm DIN, which simply applies sum pooling operations to longterm sequence embedding, in a large margin through specific designed network architecture to capture longterm user interest and tackles online serving challenge by algorithm system co-design. However, MIMN encoding all unfiltered user historical behaviors into a fixed length memories leading to it may contains lots of noise. Moreover, the memory vectors used in MIMN to represent user longterm interest is dependent on target item so that it's hard for MIMN to capture diverse long-term interest. SIM use a simple two-stage search strategy to filter out the relevant behaviors from a huge massive historical sequential behaviors and models the diverse long-term interests vary on different target items. Experiment result shows that SIM outperforms all the other long-term interest model which strongly proves that the proposed two-stage search strategy is useful for long-term user interest modeling. Moreover, as mentioned above ..., adding timestamp as position embedding achieves a further improvement.

\begin{table}
	\small
	\centering
	\caption{effectiveness evalutaion of two-stage search architecture on longterm user interest modeling}\label{tab:stage}
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{l c c}
			\addlinespace
			\toprule
			Operations on longterm behaviors        & Taobao (mean $\pm$ std) & Amazon (mean $\pm$ std)\\
			\midrule		
			{\it sum pooling without search}~ & $ 0.9006 \pm 0.00094$  &  $ 0.7411 \pm 0.00185 $  \\
			{\it only first stage (category)}~    & $ 0.9066 \pm 0.00420$  &  $ 0.7420 \pm 0.00029 $  \\
			{\it only first stage (parameter)}~    & $ 0.9081 \pm 0.00221$  &  $ 0.7481 \pm 0.00102 $  \\
			{\it SIM(first stage category)}~    & $\bm{0.9179 \pm 0.00325}$  &  $\bm{0.7593 \pm 0.00150}$  \\
			{\it SIM(first stage parameter)}~    & $\bm{0.9179 \pm 0.00325}$  &  $\bm{0.7593 \pm 0.00150}$  \\
			\bottomrule
	\end{tabular}}
\end{table}	

\subsection{Ablation Study}
\textbf{Effectiveness of the two-stage search} As mentioned above, the proposed search model uses a two-stage search strategy. 
The first stage follows a hard search strategy to filter out top-K relevant historical behaviors with target item.
%The first stage follows a rule-based hard search strategy to filter out independent historical behaviors base on categories. 
The second stage conduct an attention-based soft search on behaviors from first stage to accurately capture user's diverse long-term interest on target items.
 In this section, we will evaluate the effectiveness of the proposed two-stage search architecture by experiments with different operations applied to longterm historical behaviors. As shown in Table~\ref{tab:stage}, the first one is simply using sum pooling to integrate longterm behavior embeddings without any filters, same as long-term DIN. The second one is applying proposed first stage hard search based on categories on longterm historical behaviors and integrate filtered embeddings by sum pooling to a fixed size vectors as the input of MLP. The third one is almost the same as the second one except applying a parameter learning of search method rather than category search at the first stage. In the third experiment, we offline calculate the dot score between target item and longterm user behaviors based on pre-trained embedding vectors. The soft search is conducted by selecting top 50 relevant behaviors according to the dot score. Actually, it is a offline simulation of applying attention mechanism to longterm behavior sequences which is hard to directly serving online. And the last two experiments are the proposed search model with two-stage
serach architecture.

As shown in Table~\ref{tab:stage}, all the methods with filter strategy extremely improve model performance with simply sum pooling the embeddings. It indicates that there indeed exists massive noise in original longterm behaviors sequences which may undermine long-term user interest learning modeling. Compared with category search in first stage, offline simulated parameter search performs better. Meanwhile, we notice that there is just a little gap between the two search strategy at first stage. Obviously, the parameter search stage cost more computation and storage resources and is hard to serving online, while rule-based category search is more efficient and system friendly. Moreover, we static the search results of the two different search strategy on over 1 million samples and 100 thousands users with longterm historical behaviors from the industrial dataset. The statistical result shows that the user behaviors reserved by  hard search strategy could cover 80\% of that from the soft search strategy. Finally, we choose the simpler category search strategy at the first stage on tradeoff between efficiency and performance. Compared with models with only one stage search. The proposed search model with two-stage search strategy make a further progress by introducing attention-based search on second stage. It indicates that precisely modeling user’s diverse long-term interest on target items is helpful on CTR predict task. And after the first stage search, the filtered behavior sequences usually are much shorter than the original sequences. The attention operations wouldn't burden the online serving RTP system too much, especially with the ingeniously designed system architecture as shown in Figure 3.


\textbf{Impact of truncated length}  In the first stage, the number of top-K behaviors could inference the performance of long-term user interest modeling. In this section, we conduct experiments on SIM with different truncated length of related behaviors in the first search stage. The truncated length is manual setting as 10, 20, 50 and 100. As shown in Table ~\ref{tab:length}, in both amazon dataset and Taobao dataset experiment results proves that the model with longer relevant historical sequences preforms better. But considering the cost of experiment and final performance, we offer K set to 50. In the whole of our experiment, we fed 50 relevant behaviors to the next stage. 
%According to [], Long-term user interest
%model's performance is relevant to the length of user behavior sequences. Usually longer sequences means better performance. In this section, we conduct experiments on SIM with different truncated length of historical behaviors to verify the conclusion. The truncated length is manual setting as 200, 500, 1000 and 2000. As shown in Table ~\ref{tab:length}, in both amazon dataset and Taobao dataset, experiment results proves that the model with longer historical sequences proforms better. Meanwhile, it can be found that the performance gap between 1000 truncated length and 2000 truncated length is much smaller than that between 500 truncated length and 1000 truncated length. In other works, the influence of truncated length has marginal utility while the system latency and storage cost increase approximately linearly with the truncated length. So it's important to select suitable truncated length for specific online serving system to keep balance of system burden and model performance.

\begin{table}
	\footnotesize
	\centering
	\caption{Model performance w.r.t. different truncated length}\label{tab:length}
	\resizebox{1\columnwidth}{!}{%
		\begin{tabular}{l c c}
			\addlinespace
			\toprule
		~~~~	truncated length        ~~~~       & Taobao (mean $\pm$ std) &Amazon (mean $\pm$ std) \\
			\midrule
		~~~~	{\it 10}     ~~~~     & $ 0.9046 \pm 0.00135 $  &  $ \bm{0.7522 \pm 0.00231}$  \\
		~~~~	{\it 20}      ~~~~    & $ 0.9052 \pm 0.00202 $  &  $ 0.7503 \pm 0.00120$   \\
		~~~~	{\it 50}      ~~~~    & $ \bm{0.9070 \pm 0.00186} $  &  $ 0.7486 \pm 0.00071$  \\
		~~~~	{\it 100}      ~~~~    & $ \bm{0.9070 \pm 0.00186} $  &  $ 0.7486 \pm 0.00071$  \\
			\bottomrule
	\end{tabular}}
\end{table}


\begin{table}
		\tiny
        \centering
        \caption{Model performance (AUC) on industrial dataset}\label{tab:deploy}
        \resizebox{\columnwidth}{!}{%
                \begin{tabular}{l cc}
                        \addlinespace
                        \toprule
                     ~~~~~   Model ~~~~~  &AUC      ~~~~~ \\
                        \midrule
                     ~~~~~   {\it MIMN} ~~~~~& $0.6541$  ~~~~~\\
                     ~~~~~   {\it SIM} ~~~~~& $0.6604$     ~~~~~ \\
                     ~~~~~   {\it SIM with timestamp } ~~~~~&$0.6624 $ ~~~~~\\
                        \bottomrule
        \end{tabular}}
\end{table}

\subsection{Results on Industrial Dataset}
We further conduct experiments on the dataset collected from online display advertisement system of Alibaba. We compared SIM with the model of MIMN. Table~\ref{tab:deploy} shows the results. SIM improves MIMN with AUC gain of 0.008, which is significant for our business. 

\textbf{Online A/B Testing.} 
We have deployed the proposed solution in the display advertising system in Alibaba. 
From 2020-02-20 to 2020-04-20, we conduct strict online A/B testing experiment to validate the proposed SIM model. 
Compared to MIMN (our last product model), SIM achieves 7.5\% CTR and 4\% RPM (Revenue Per Mille) gain.
Now, SIM has been deployed online and serves the main scene traffic, which contributes a significant business revenue growth.

%It is worth noticing that online serving of DIEN is a great challenge for commercial system. Online system holds re- ally high traffic in our display advertising system, which serves more than 1 million users per second at traffic peak. In order to keep low latency and high throughput, we de- ploy several important techniques to improve serving per- formance: i) element parallel GRU & kernel fusion (Wang, Lin, and Yi 2010), we fuse as many independent kernels as possible. Besides, each element of the hidden state of GRU can be calculated in parallel. ii) Batching: adjacent requests from different users are merged into one batch to take advantage of GPU. iii) Model compressing with Rocket Launching (Zhou et al. 2018b): we use the method proposed in (Zhou et al. 2018b) to train a light network, which has smaller size but performs close to the deeper and more com- plex one. For instance, the dimension of GRU hidden state can be compressed from 108 to 32 with the help of Rocket Launching. With the help of these techniques, latency of DIEN serving can be reduced from 38.2 ms to 6.6 ms and the QPS (Query Per Second) capacity of each worker can be improved to 360.

\textbf{Rethinking Search Model.} 

\textbf{Practical Experience For Deployment.}
It is worth noticing that online serving of SIM is a great challenge for real-time CTR prediction system. High traffic in Alibaba display advertising system is well-known, which serves more than 1 million users per second at traffic peak. Previous works each request contain a copy of user features. But at SIM, user features expand 
Dozens of times due to the diverse user behaviors with different target ads. The computation and bandwidth would increase with the user features. Taking advantage of recommendation system characteristic, 90\% diverse user behaviors can be compressed. we take the distinct of diverse user behaviors with target category and an indicator table to conduct.  At the same time, the diverse user behaviors cause the computation of attention could not transform to matrix multiply operation. The diverse user behaviors would be gathered in attention score computation. We optimize the computation of multi-head scores to parallel and reduce the latency of calculation.
Our real-time CTR prediction system system performance of latency and GPU utilization with MIMN and SIM shows in Figure [ref].


% % since 2019.01.26 in the display advertising system of Alibaba. Unfortunately, it is close to the Spring Festival of China and users are not active during this period, making the result of online  A/B testing to be not reliable. We will show the comparison result in later camera ready version if accepted.

% % In the online display advertising system, we can record the history behavior for a long time. In Figure\ref{fig:length}, we can find the long sequence is a universal phenomena in industrial scene. So when we want to model the periodical item prediction, we need to involve the history behavior for a long time. We can find the effect of our model gradually better when the length of user behavior is growing. For comparing the length of behavior sequence, we remove some aggregation feature.

% % \begin{figure}[!htb]
% % 	\centering
% % 	\includegraphics[width=8.6cm]{./length.pdf}
% % 	\caption{The length of user behavior sequence in different days and the effect to model different length of behavior sequence}
% % 	\label{fig:length}
% % \end{figure}

% \begin{figure}[!htb]
% 	\centering
% 	\includegraphics[width=8.5cm]{./qps.pdf}
% 	\caption{System performance of realtime CTR prediction system w.r.t. different length of user behavior sequences, serving with MIMN and DIEN model. MIMN model is implemented with the design of UIC server.}
% 	\label{fig:qps}
% \end{figure}

% \subsection{Practical Experience For Deployment} 
% In this section, we discuss practical experience on deploying the proposed solution of UIC and MIMN in our online system. 


% \textbf{Synchronization of UIC Server and RTP Server}.
% As is introduced in section , MIMN is implemented with UIC and RTP servers together. Hence there is an out-sync problem between UIC and RTP server. Asynchronous parameter update of the two servers might cause incorrect model inference in real systems with periodic model deployment, which is of great risk. Experiment is conducted to simulate the out-sync situation. Table  shows the results. MIMN with out-sync parameter update shows little difference on model performance. Note in this experiment, the gap of out-sync update time is within one day, which is a traditional setting in industrial systems. Actually in our real system, model deployment is designed to be executed hourly, reducing the risk further. We believe this is due to the stable representation of user interests that MIMN learned, resulting in good generalization performance of MIMN.            

% \textbf{The Influence of Big-Sale Data}.
% Nowadays, big sale is adopted by many e-commerce sites to attract customers for online consumption, e.g. the famous 11.11 big sale of Alibaba in China. In this extreme situation, the distribution of sample as well as user behaviors are quite different from that in daily situation. We compare the the performance of MIMN with and without training data collected at the big sale day of 11.11 in our system. The results are shown in Table. We find it's better to remove the big-sale data empirically. 
    
% \textbf{Warm Up Strategy}.
% Although UIC is designed to update incrementally, it will take a fairly long time for stable accumulation from the beginning. Practically, we employ the warm up strategy to initialize UIC with pre-calculated user interest representations. That is, we collect historical behaviors of last 120 days (with average length of user behavior sequences to be 1000) for each user and make inference with trained MIMN model in an offline mode, then push the accumulated memories into UIC for further incremental update. This strategy enables a reasonable model performance when deploying the proposed solution as soon as possible.      

% \textbf{Rollback Strategy}. 
% In case with unexpected problem, e.g. pollution of training samples by large-scale online cheating, the incremental update mechanism of UIC server may suffer a lot. A troublesome challenge is to seek to the point where abnormal case happened. To defend against this risk, we design a rollback strategy that stores the copy of learned user interest representation at 00:00 am every day and record that of the last 7 days.     






